The pde2path add-on toolbox p2pOC for solving infinite time-horizon spatially distributed optimal control problems - Quickstart Guide -

p2pOC is an add-on toolbox to the Matlab package pde2path. It is aimed at the numerical solution of optimal control (OC) problems with an infinite time horizon for parabolic systems of PDE over 1D or 2D spatial domains. The basic idea is to treat the OC problem via the associated canonical system in two steps. First we use pde2path to find branches of stationary solutions of the canonical system, also called canonical steady states (CSS). In a second step we use the results and the spatial discretization of the first step to calculate the objective values of time-dependent canonical paths ending at a CSS with the so called saddle point property. This is a (typically very high dimensional) boundary value problem (BVP) in time, which we solve by combining a modification of the BVP solver TOM with a continuation algorithm in the initial states. We explain the design and usage of the package via two example problems, namely the optimal management of a distributed shallow lake model, and of a semi-arid grazing system. Both show interesting bifurcations of so called patterned CSS, and in particular the latter also a variety of patterned optimal steady states. The package (library and demos) can be downloaded at www.staff.uni-oldenburg.de/hannes.uecker/pde2path.

==> slsource1.tex <==

\begin{table}[!ht]
{\small%\footnotesize
\begin{tabular}{|p{0.98\textwidth}|}
\hline\\\vs{-10mm}
\begin{verbatim}
function p=slinit(p,lx,ly,nx,ny,sw) % init-routine 
p=stanparam(p); % set generic parameters to standard, if needed reset below..
p.nc.neq=2; p.fuha.G=@slf; p.fuha.Gjac=@sljac; p.fuha.outfu=@ocbra; % rhs 
p.fuha.sG=@slsG; p.fuha.sGjac=@slsGjac; p.fuha.jcf=@sljcf; % current-val-obj 
pre=sprintf('%s',inputname(1)); p=setfn(p,pre);            % filename  
p.usrlam=[0.55 0.6 0.65 0.7 0.75]; % target-values for lam 
[p.mesh.geo,bc]=recnbc2(lx,ly); p.vol=4*lx*ly; % geometry, and volume of dom 
p.fuha.bc=@(p,u) bc; p.fuha.bcjac=@(p,u) bc;   % standard Neumann BC 
p.xplot=lx; p.sw.spcalc=0; p.sw.jac=1; p.file.smod=100; % some more switches 
par=[0.03;0.55;0.5;0.5]; p.nc.ilam=2; p.sol.ds=0.1;   % startup param 
% rho=par(1); bp=par(2); cp=par(3); D=par(4); 
p.nc.dsmin=1e-6; p.nc.dsmax=0.5; p.nc.lammax=0.8; p.nc.lammin=0.549; 
p=stanmesh(p,nx,ny);p=setbmesh(p); p.sol.xi=1/p.np;   % mesh 
p.eqn.c=[1;0;0;1;-1;0;0;-1]; p.eqn.a=0; p.eqn.b=0;    % diffusion tensor 
switch sw  % choose initial guess arcoording to switch 
case 1; u=0.3*ones(p.np,1); v=-13*ones(p.np,1); u0=[u v]; p.u=u0(:); % FSC
case 2; u=2*ones(p.np,1); v=-4*ones(p.np,1); u0=[u v]; p.u=u0(:); % FSM
case 3; u=3*ones(p.np,1); v=-4*ones(p.np,1); u0=[u v]; p.u=u0(:); 
    par=[0.3;0.55;2.5;0.5]; p.nc.ilam=3; % Scenario 2
    p.nc.lammax=3.7; p.nc.lammin=2.5; p.usrlam=3.25;
end
p.u=[p.u; par]; p.sw.sfem=1; p=setfemops(p);  % semilin. setting 
[p.u,res]=nloop(p,p.u); fprintf('first res=%g\n',res); plotsol(p,1,1,1); 
\end{verbatim}
\vs{-8mm}
\\\hline\hline\\\vs{-10mm}
\begin{verbatim}
function r=slsG(p,u) % SL p_t=D*lap p-1/q-b*p+p^2/(1+p^2)
%                         q_t=-D lap q+2cp*p+q*(rho+bp-2*p/(1+p^2)^2; 
par=u(p.nu+1:end); rho=par(1); bp=par(2); cp=par(3); D=par(4); 
P=u(1:p.np); q=u(p.np+1:2*p.np); 
f1=-1./q-bp*P+p.^2./(1+P.^2); f2=2*cp*P+q.*(rho+bp-2*p./(1+P.^2).^2); 
f=[f1;f2]; r=D*p.mat.K*u(1:p.nu)-p.mat.M*f; 
\end{verbatim}\vs{-8mm}\\\hline\hline  \vs{-5mm}
\begin{verbatim}
function jc=sljcf(p,u) % current value J for slOC
par=u(p.nu+1:end); cp=par(3); pv=u(1:p.np); kv=-1./u(p.np+1:p.nu); jc=log(kv)-cp*pv.^2;
\end{verbatim}
\vs{-8mm}\\\hline
\end{tabular}}
\vs{0mm}
\caption{{\small The init routine {\tt slinit.m}, the rhs {\tt slsG.m}, 
and the objective function {\tt sljcf.m}. See also, 
e.g.,  the source code 
of {\tt slsGjac} for the implementation of $G_u$. }\label{tab4}}\end{table}



 

==> slsource2.tex <==
\begin{table}[!ht]
{\small%\footnotesize
\begin{tabular}{p{0.98\textwidth}}
\hline\\\vs{-8mm}
\begin{verbatim}
%% stat. BD for sloc, main script-file. First set matlab paths: 
path('../p2plib',path);path('../oclib',path);
\end{verbatim}\vs{-5mm}\rule{4cm}{0.4pt}\vs{-3mm}\begin{verbatim}
%% Scenario 1, FSC/FSI branch 
close all; p=[];lx=2*pi/0.44; ly=0.1; nx=50; ny=1; sw=1; p=slinit(p,lx,ly,nx,ny,sw); 
p=setfn(p,'f1'); screenlayout(p); p=cont(p,100); 
\end{verbatim}\vs{-5mm}\rule{4cm}{0.4pt}\vs{-3mm}\begin{verbatim}
%% FSM branch 
sw=2; p=slinit(p,lx,ly,nx,ny,sw); p=setfn(p,'f2'); p.nc.dsmax=0.2; p=cont(p,15); 
\end{verbatim}\vs{-5mm}\rule{4cm}{0.4pt}\vs{-3mm}\begin{verbatim}
%% bif from f1 (set bpt* and p* and repeat as necessary) 
p=swibra('f1','bpt1','p1',-0.05); p.nc.dsmax=0.3; p.nc.neigdet=50; p=cont(p,150); 
\end{verbatim}\vs{-5mm}\rule{4cm}{0.4pt}\vs{-3mm}\begin{verbatim}
%% plotting of BD, L2
clf(3); pcmp=3; plotbraf('f1','bpt1',3,pcmp,'lab',12,'cl','k'); % FSC (+ other branches) 
\end{verbatim}\vs{-5mm}\rule{4cm}{0.4pt}\vs{-3mm}\begin{verbatim}
%% plotting of BD, J_{ca}
clf(3); pcmp=4; plotbraf('f1','bpt1',3,pcmp,'lab',12,'cl','k'); % FSC (+other branches)
\end{verbatim}\vs{-5mm}\rule{4cm}{0.4pt}\vs{-3mm}\begin{verbatim}
plot1Df('p1','pt16',1,1,1,2); plot1Df('p1','pt71',2,1,1,2); % solution plots ...
\end{verbatim}
\vs{-6mm}\\\hline
\end{tabular}}
\vs{0mm}
\caption{{\small Selected commands from the script file {\tt bdcmds.m}. 
The horizontal lines seperate the different cells of that file, which 
should be executed one by one. 
See the source code for more details, and, e.g., {\tt bdcmds2D.m} 
for the quite similar commands in 2D. }\label{tab4b}}\end{table}

==> slsource3.tex <==
\begin{table}[!ht]
{\footnotesize
\begin{tabular}{p{0.98\textwidth}}
\hline\\\vs{-8mm}
\begin{verbatim}
% driver script for Shallow Lake Optimal Control 
path('../tom',path); % assuming p2plib and oclib paths are already set 
close all; clear all; global s0 s1 u0 u1 Psi par xi ym1 ym2 sig;  
\end{verbatim}\vs{-5mm}\rule{4cm}{0.4pt}\vs{-3mm}\begin{verbatim}
%% ---- Fig2a, Preparations: put filenames into fn, set some bvp parameters 
fn.sd1='f1'; fn.sp1='pt12'; fn.sd0='p3'; fn.sp0='pt19'; 
opt=tomset('FJacobian',@fjac,'BCJacobian',@cbcjac); opt.lusw=0; ...;  opt.nti=10; 
\end{verbatim}\vs{-5mm}\rule{4cm}{0.4pt}\vs{-3mm}\begin{verbatim}
%% the solve and continue call, and some plots 
alvin=[0.25 0.5 0.75 1]; ti1=tic; [alv,vv,sol,ydat]=isctr(alvin,opt,fn); ti1=toc(ti1)
zdia=sldiagn(sol,15); psol3D(s1,sol,1,1,'P'); clf(6); plot(alv(1,:),vv(1,:),'-*'); 
\end{verbatim}\vs{-5mm}\rule{4cm}{0.4pt}\vs{-3mm}\begin{verbatim}
%% ---- Fig4a, here iscarc needed. Preparations and initial iscarc-call: 
fn.sd1='f1'; fn.sp1='pt12'; fn.sd0='p1'; fn.sp0='pt71'; esol=[]; ysec=[]; 
opt.nsteps=3; opt.alvin=[0.2 0.25]; sig=0.1;...; opt.start=1;  
[alv,vv,ysec1,esol1,tlv,xv,yv]=iscarc(esol,ysec,opt,fn); opt.start=0; 
\end{verbatim}\vs{-5mm}\rule{4cm}{0.4pt}\vs{-3mm}\begin{verbatim}
%% subsequent iccarc-calls: 
opt.nsteps=20; ysec=ysec1; esol=esol1; % new input (for repeated calls) 
[alv1,vv1,ysec1,esol1,tlv1,xv1,yv1]=iscarc(esol,ysec,opt,fn); 
% append output to prev. steps for repeated calls 
alv=[alv alv1]; vv=[vv vv1]; tlv=[tlv tlv1]; xv=[xv; xv1]; yv=[yv; yv1]; 
\end{verbatim}\vs{-5mm}\rule{4cm}{0.4pt}\vs{-3mm}\begin{verbatim}
%% select and postprocess solution from iscarc (here the 5th) 
j=5; tl=tlv(j); n=s1.nu; sol.x=xv(j,1:tlv(j)); sol.y=squeeze(yv(j,1:n,1:tlv(j)));
al=alv(j), u0=al*s0.u(1:n)+(1-al)*s1.u(1:n); u1=s1.u(1:s1.nu); % some plots:
zdia=sldiagn(sol,15); psol3D(s1,sol,1,1,'P'); psol3D(s1,sol,2,2,'k'); 
\end{verbatim}
\vs{-6mm}\\\hline
\end{tabular}}
\vs{0mm}
\caption{{\small Selected commands from the script file {\tt cpdemo.m}. 
See the source code for more details and, e.g., more fancy 
plotting. }\label{tab7}}\end{table}
